Double-Directional Information Azimuth Spectrum and Relay Network Tomography for a Decentralized Wireless Relay Network

A novel channel representation for a two-hop decentralized wireless relay network (DWRN) is proposed, where the relays operate in a completely distributive fashion. The modeling paradigm applies an analogous approach to the description method for a double-directional multipath propagation channel, and takes into account the finite system spatial resolution and the extended relay listening/transmitting time. Specifically, the double-directional information azimuth spectrum (IAS) is formulated to provide a compact representation of information flows in a DWRN. The proposed channel representation is then analyzed from a geometrically-based statistical modeling perspective. Finally, we look into the problem of relay network tomography (RNT), which solves an inverse problem to infer the internal structure of a DWRN by using the instantaneous doubledirectional IAS recorded at multiple measuring nodes exterior to the relay region.

==> IEEEbib.tex <==
% ------------------------------------------------------------------------
% SAMPLE BIBLIOGRAPHY FILE
% ------------------------------------------------------------------------

@BOOK{PNG03,
   author = "A. Paulraj, R. Nabar, and D. Gore",
   title= "Introduction to Space-Time Wireless Communications",
   publisher = "Cambridge University Press",
   year = 2003
}

@BOOK{VA04,
   author = "R. Vaughan and J. B. Andersen",
   title= "Channels, Propagation and Antennas for Mobile Communications",
   publisher = "The Institute of Electrical Engineering",
   year = 2004
}

@ARTICLE{GBGP02,
 author={D. Gesbert, H. Bölcskei, D. A. Gore, and A. J. Paulraj},
 title={Outdoor MIMO wireless channels: models and performance prediction},
 journal={IEEE J. Select. Areas Commun.},
 volume={50},
 number={12},
 year={2002},
 pages={1926-1934},
}

@ARTICLE{AMS02,
 author={A. M. Sayeed},
 title={Deconstructing multi-antenna fading channels},
 journal={IEEE Trans. Signal Processing},
 volume={50},
 year={2002},
 pages={2563-2579},
}

@ARTICLE{PH03,
 author={A. Poon and M. Ho},
 title={Indoor multiple-antenna channel characterization from 2 to 8 GHz},
 journal={Proceedings of IEEE ICC2003},
 year={2003},
 volume={5}
 pages={3519-3523}
}

@BOOK{CAB97,
   author = "C. A. Balanis",
   title= "Antenna Theory: Analysis and Design",
   publisher = "John Wiley & Sons",
   year = 1997
}

@ARTICLE{JPR99,
 author={J-P Rossi},
 title={Influence of measurement conditions on the evaluation of some radio channel parameters},
 journal={IEEE Trans. Veh. Technol.},
 volume={48},
 year={1999},
 pages={1304-1316},
}

